plingo: A system for probabilistic reasoning in clingo based on lpmln

We present plingo, an extension of the ASP system clingo with various probabilistic reasoning modes. Plingo is centered upon LP^MLN, a probabilistic extension of ASP based on a weight scheme from Markov Logic. This choice is motivated by the fact that the core probabilistic reasoning modes can be mapped onto optimization problems and that LP^MLN may serve as a middle-ground formalism connecting to other probabilistic approaches. As a result, plingo offers three alternative frontends, for LP^MLN, P-log, and ProbLog. The corresponding input languages and reasoning modes are implemented by means of clingo's multi-shot and theory solving capabilities. The core of plingo amounts to a re-implementation of LP^MLN in terms of modern ASP technology, extended by an approximation technique based on a new method for answer set enumeration in the order of optimality. We evaluate plingo's performance empirically by comparing it to other probabilistic systems.

==> macro.tex <==
%\newcommand{\lpmln}{\ensuremath{\mathit{LP}^{\mathit{MLN}}}}
%\newcommand{\lpmln}{\ensuremath{\mathit{Lpmln}}}
\newcommand{\lpmln}{\textit{Lpmln}}
\newcommand{\plog}{\textit{P-log}}
\newcommand{\problog}{\textit{ProbLog}}
%\newcommand{\lpmlnl}{\ensuremath{\mathit{LP}^{\mathit{MLN}}}}
%\newcommand{\lpmlnl}{\ensuremath{\mathit{Lpmln}}}
\newcommand{\lpmlnl}{\textit{Lpmln}}
%\renewcommand{\plingo}{\ensuremath{\mathit{LP}^{\mathit{MLN\pm}}}}
%\renewcommand{\plingo}{\ensuremath{\mathit{Lpmln}^{\mathit{\pm}}}}
\renewcommand{\plingo}{\textit{Lpmln}\ensuremath{^{\mathit{\pm}}}}
\newcommand{\smproblog}{\textit{SMProblog}}

\newcommand{\sclingo}{\textit{clingo}}
\newcommand{\Splingo}{\textit{Plingo}}
\newcommand{\splingo}{\textit{plingo}}
\newcommand{\slpmln}{\textit{lpmln2asp}}
\newcommand{\splog}{\textit{plog}}
\newcommand{\splognaive}{\textit{plog-naive}}
\newcommand{\splogdco}{\textit{plog-dco}}
\newcommand{\sproblog}{\textit{problog}}
\newcommand{\saspmc}{\textit{aspmc}}

\newcommand{\unw}[1]{\ensuremath{{\overline{#1}}}}
\newcommand{\norm}[1]{\ensuremath{{{#1}^*}}}
\newcommand{\sm}[1]{\ensuremath{\mathit{SM}(#1)}}
\newcommand{\ssm}[1]{\ensuremath{\mathit{SSM}(#1)}}
\newcommand{\ssmp}[1]{\ensuremath{\mathit{SSM}^{\mathit{alt}}(#1)}}
% \newcommand{\osm}[1]{\ensuremath{\mathit{OSM}^{{\pm}}(#1)}}
\newcommand{\osm}[1]{\ensuremath{\mathit{OPT}^{{\pm}}(#1)}}
\newcommand{\os}[1]{\ensuremath{\mathit{OS}^{{\pm}}(#1)}}
\newcommand{\nos}[1]{\ensuremath{\mathit{NOS}^{{\pm}}(#1)}}

\newcommand{\tw}[1]{\ensuremath{\mathit{TW}(#1)}}
\newcommand{\sumw}[1]{\ensuremath{\mathit{SUMW}(#1)}}
\newcommand{\sumwp}[1]{\ensuremath{\mathit{SUMW}'(#1)}}
\newcommand{\sumwpp}[1]{\ensuremath{\mathit{SUMW}''(#1)}}
\newcommand{\sumwplingo}[1]{\ensuremath{\mathit{SUMW}'''(#1)}}
\newcommand{\osmplingo}[1]{\ensuremath{\mathit{OSM}^{\mathit{plingo}}(#1)}}

\newcommand{\weight}[2]{\ensuremath{W_{#1}(#2)}}
\newcommand{\weightp}[2]{\ensuremath{W_{#1}^{\mathit{alt}}(#2)}}
\newcommand{\weightpp}[2]{\ensuremath{W_{#1}^{{\pm}}(#2)}}
\newcommand{\weightplingo}[2]{\ensuremath{W_{#1}^{\mathit{plingo}}(#2)}}

\newcommand{\prob}[2]{\ensuremath{P_{#1}(#2)}}
\newcommand{\probbasic}[2]{\ensuremath{P^{\mathit{basic}}_{#1}(#2)}}
\newcommand{\probp}[2]{\ensuremath{P_{#1}^{\mathit{alt}}(#2)}}
\newcommand{\probpp}[2]{\ensuremath{P_{#1}^{{\pm}}(#2)}}
\newcommand{\probplingo}[2]{\ensuremath{P_{#1}^{\mathit{plingo}}(#2)}}

\newcommand{\soft}[1]{\ensuremath{#1^{\mathit{soft}}}}
\newcommand{\hard}[1]{\ensuremath{#1^{\mathit{hard}}}}
\newcommand{\weak}[1]{\ensuremath{#1^{\mathit{weak}}}}
\newcommand{\transone}[1]{\ensuremath{#1^{*}}}
%\newcommand{\transtwo}[1]{\ensuremath{#1^{\star}}}
\newcommand{\transtwo}[1]{\ensuremath{\mathit{standard}(#1)}}
\newcommand{\transtwozero}[0]{\ensuremath{\mathit{standard}}}
%\newcommand{\transthree}[1]{\ensuremath{#1^{\bullet}}}
\newcommand{\transthree}[1]{\ensuremath{\mathit{alternative}(#1)}}
\newcommand{\transthreezero}[0]{\ensuremath{\mathit{alternative}}}
%\newcommand{\transthree}[1]{\ensuremath{#1^{\bullet}}}
%\newcommand{\transfour}[1]{\ensuremath{#1'}}
\newcommand{\transfour}[1]{\ensuremath{\mathit{negative}(#1)}}
\newcommand{\transtwoname}[1]{\ensuremath{\star}}
\newcommand{\transthreename}[1]{\ensuremath{\bullet}}

\newcommand{\totalcost}[2]{\ensuremath{\mathit{Cost}_{#1}(#2)}}
\newcommand{\cost}[3]{\ensuremath{\mathit{Cost}_{#1}(#2,#3)}}
\newcommand{\costplingo}[2]{\ensuremath{\mathit{Cost}_{#1}(#2,0)}}

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newcommand{\qed}{QED}
\newenvironment{proofof}[1]{\noindent {\bf Proof of #1.}}{\qed}

% Problog
\newcommand{\problognormal}[1]{\ensuremath{{{#1}^{\mathit{normal}}}}}
\newcommand{\problognormalsub}[2]{\ensuremath{{{#1}_{#2}^{\mathit{normal}}}}}
%\newcommand{\problogfacts}[1]{\ensuremath{{{#1}^{\mathit{facts}}}}}
\newcommand{\problogfacts}[1]{\ensuremath{{{#1}^{\mathit{probs}}}}}
\newcommand{\problogfactssub}[2]{\ensuremath{{{#1}_{#2}^{\mathit{probs}}}}}
\newcommand{\problogevidence}[1]{\ensuremath{{{#1}^{\mathit{evidence}}}}}
%\newcommand{\problogatoms}[1]{\ensuremath{{{#1}^{\mathit{atoms}}}}}
\newcommand{\problogatoms}[1]{\ensuremath{{{\mathit{choices}(#1)}}}}
\newcommand{\problogatomssub}[2]{\ensuremath{{{\mathit{choices}(#1_#2)}}}}
\newcommand{\problogtolpmlnzero}[0]{\ensuremath{{{\mathit{problog2lpmln}}}}}
\newcommand{\problogtolpmln}[1]{\ensuremath{{{\mathit{problog2lpmln}(#1)}}}}
\newcommand{\lpmlntoproblog}[1]{\ensuremath{{{\mathit{lpmln2problog}(#1)}}}}
\newcommand{\lpmlntoproblogzero}[0]{\ensuremath{{{\mathit{lpmln2problog}}}}}
\newcommand{\pnf}[0]{\ensuremath{{{\mathit{PNF}}}}}
\newcommand{\tr}[1]{\ensuremath{{\mathit{stratify}}(#1)}}
%\newcommand{\posa}[1]{\ensuremath{#1^{+}}}
\newcommand{\posa}[1]{\ensuremath{#1'}}
%\newcommand{\posa}[1]{\ensuremath{#1^{\bullet}}}
\newcommand{\nega}[1]{\ensuremath{#1^{-}}}
\newcommand{\mybot}[0]{\ensuremath{\mathit{bot}}}
\newcommand{\copya}[1]{\ensuremath{\mathit{copy}(#1)}}
\newcommand{\atoms}[1]{\ensuremath{\mathit{atoms}(#1)}}
\newcommand{\softatoms}[1]{\ensuremath{\mathit{soft}(#1)}}

% Problog proofs
% \newcommand{\pione}[0]{\mathit{tr}_1(\Pi)}
\newcommand{\pione}[0]{\Pi_1}
% \newcommand{\pitwo}[0]{\mathit{tr}_2(\Pi)}
\newcommand{\pitwo}[0]{\Pi_2}
\newcommand{\pifinal}[0]{\problogtolpmln{\Pi}}
\newcommand{\pifinalnoev}[0]{\problogtolpmln{\Pi\setminus\problogevidence{\Pi}}}
\newcommand{\pifinalproblog}[0]{\Pi\setminus\problogevidence{\Pi}}
\newcommand{\ssum}[1]{\ensuremath{\mathit{sum}(#1)}}
\newcommand{\problogmodels}[1]{\ensuremath{\mathit{models}(#1)}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

